Polycyclic Aromatic Hydrocarbon and CO(2-1) Emission at 50-150 pc Scales in 70 Nearby Galaxies

Combining Atacama Large Millimeter/sub-millimeter Array CO(2-1) mapping and JWST near- and mid-infrared imaging, we characterize the relationship between CO(2-1) and polycyclic aromatic hydrocarbon (PAH) emission at ~100 pc resolution in 70 nearby star-forming galaxies. Leveraging a new Cycle 2 JWST treasury program targeting nearby galaxies, we expand the sample size by more than an order of magnitude compared to previous ~100 pc resolution CO-PAH comparisons. Focusing on regions of galaxies where most of the gas is likely to be molecular, we find strong correlations between CO(2-1) and 3.3 um, 7.7 um, and 11.3 um PAH emission, estimated from JWST's F335M, F770W, and F1130W filters. We derive power law relations between CO(2-1) and PAH emission, which have indices in the range 0.8-1.3, implying relatively weak variations in the observed CO-to-PAH ratios across the regions that we study. We find that CO-to-PAH ratios and scaling relationships near HII regions are similar to those in diffuse sight lines. The main difference between the two types of regions is that sight lines near HII regions show higher intensities in all tracers. Galaxy centers, on the other hand, show higher overall intensities and enhanced CO-to-PAH ratios compared to galaxy disks. Individual galaxies show 0.19 dex scatter in the normalization of CO at fixed I_PAH, and this normalization anti-correlates with specific star formation rate (sSFR) and correlates with stellar mass. We provide a prescription that accounts for these galaxy-to-galaxy variations and represents our best current empirical predictor to estimate CO(2-1) intensity from PAH emission, which allows one to take advantage of JWST's excellent sensitivity and resolution to trace cold gas.

==> gal_table.tex <==
\startlongtable
\begin{deluxetable*}{lrrrrrrrrr}
\label{tab:galtab}
\tablecolumns{9}
\tablecaption{Fits to all pixels outside galaxy centers for each galaxy.}
\tablehead{
\colhead{Name} & \colhead{Cycle} & \colhead{$\log_{10}M_\star$} & \colhead{$\log_{10}\mathrm{SFR}/M_\star$} & \colhead{$m$} & \colhead{$b$} & \colhead{$x_0$} & \colhead{$\log_{10}C_\mathrm{band}$} & \colhead{$N_\mathrm{pix}$} & \colhead{$r$}}
\startdata
\cutinhead{$I_\mathrm{CO(2-1)}$ vs F770W$_\mathrm{PAH}$}
IC5273 & 2 & $9.72$ & $-9.99$ & $0.941 \pm 0.215$ & $0.217 \pm 0.090$ & $0.517$ & $-0.269$ & $19065$ & $0.68$ \\
IC5332 & 1 & $9.68$ & $-10.07$ & $0.415 \pm 0.866$ & $0.352 \pm 0.270$ & $0.375$ & $0.197$ & $6748$ & $0.18$ \\
NGC0628 & 1 & $10.34$ & $-10.10$ & $0.697 \pm 0.294$ & $0.591 \pm 0.116$ & $0.517$ & $0.231$ & $11989$ & $0.54$ \\
NGC1087 & 1 & $9.94$ & $-9.83$ & $1.174 \pm 0.188$ & $0.614 \pm 0.102$ & $0.801$ & $-0.326$ & $9201$ & $0.72$ \\
NGC1097 & 2 & $10.76$ & $-10.08$ & $0.755 \pm 0.213$ & $0.674 \pm 0.097$ & $0.588$ & $0.230$ & $55013$ & $0.61$ \\
NGC1300 & 1 & $10.62$ & $-10.55$ & $0.897 \pm 0.492$ & $0.508 \pm 0.169$ & $0.446$ & $0.109$ & $3665$ & $0.46$ \\
NGC1365 & 1 & $11.00$ & $-9.76$ & $1.299 \pm 0.335$ & $0.803 \pm 0.178$ & $0.588$ & $0.040$ & $9512$ & $0.39$ \\
NGC1385 & 1 & $9.98$ & $-9.66$ & $1.034 \pm 0.175$ & $0.584 \pm 0.112$ & $0.872$ & $-0.318$ & $10653$ & $0.74$ \\
NGC1433 & 1 & $10.87$ & $-10.82$ & $1.248 \pm 0.501$ & $0.576 \pm 0.165$ & $0.446$ & $0.020$ & $6738$ & $0.40$ \\
NGC1511 & 2 & $9.91$ & $-9.55$ & $0.895 \pm 0.117$ & $0.559 \pm 0.068$ & $0.801$ & $-0.158$ & $14424$ & $0.82$ \\
NGC1512 & 1 & $10.72$ & $-10.61$ & $0.900 \pm 0.623$ & $0.377 \pm 0.160$ & $0.304$ & $0.104$ & $3243$ & $0.48$ \\
NGC1546 & 2 & $10.35$ & $-10.43$ & $0.824 \pm 0.092$ & $0.753 \pm 0.044$ & $0.659$ & $0.210$ & $9933$ & $0.96$ \\
NGC1559 & 2 & $10.36$ & $-9.79$ & $0.947 \pm 0.150$ & $0.519 \pm 0.083$ & $0.801$ & $-0.239$ & $42127$ & $0.76$ \\
NGC1566 & 1 & $10.79$ & $-10.13$ & $1.003 \pm 0.192$ & $0.826 \pm 0.121$ & $0.872$ & $-0.048$ & $28064$ & $0.60$ \\
NGC1637 & 2 & $9.95$ & $-10.14$ & $0.791 \pm 0.223$ & $0.548 \pm 0.092$ & $0.588$ & $0.083$ & $39895$ & $0.67$ \\
NGC1672 & 1 & $10.73$ & $-9.85$ & $1.239 \pm 0.263$ & $0.733 \pm 0.128$ & $0.730$ & $-0.170$ & $8946$ & $0.64$ \\
NGC1792 & 2 & $10.61$ & $-10.04$ & $0.852 \pm 0.115$ & $0.780 \pm 0.068$ & $0.872$ & $0.037$ & $59996$ & $0.86$ \\
NGC1809 & 2 & $9.77$ & $-9.01$ & $0.977 \pm 0.440$ & $0.230 \pm 0.130$ & $0.375$ & $-0.136$ & $6042$ & $0.58$ \\
NGC2090 & 2 & $10.04$ & $-10.43$ & $0.639 \pm 0.325$ & $0.392 \pm 0.108$ & $0.375$ & $0.153$ & $13045$ & $0.66$ \\
NGC2283 & 2 & $9.89$ & $-10.17$ & $0.948 \pm 0.258$ & $0.289 \pm 0.108$ & $0.588$ & $-0.269$ & $26689$ & $0.58$ \\
NGC2566 & 2 & $10.71$ & $-9.77$ & $0.907 \pm 0.293$ & $0.611 \pm 0.122$ & $0.588$ & $0.078$ & $34275$ & $0.56$ \\
NGC2775 & 2 & $11.07$ & $-11.13$ & $0.694 \pm 0.300$ & $0.492 \pm 0.094$ & $0.375$ & $0.232$ & $26633$ & $0.56$ \\
NGC2835 & 1 & $10.00$ & $-9.90$ & $0.936 \pm 0.424$ & $0.380 \pm 0.161$ & $0.517$ & $-0.104$ & $10158$ & $0.39$ \\
NGC2903 & 2 & $10.63$ & $-10.15$ & $0.844 \pm 0.136$ & $0.709 \pm 0.083$ & $0.801$ & $0.034$ & $119478$ & $0.74$ \\
NGC2997 & 2 & $10.73$ & $-10.09$ & $0.773 \pm 0.115$ & $0.864 \pm 0.077$ & $0.943$ & $0.135$ & $223223$ & $0.67$ \\
NGC3059 & 2 & $10.38$ & $-10.00$ & $1.014 \pm 0.107$ & $0.934 \pm 0.078$ & $1.085$ & $-0.167$ & $59783$ & $0.66$ \\
NGC3137 & 2 & $9.88$ & $-10.19$ & $0.574 \pm 1.485$ & $0.140 \pm 0.294$ & $0.233$ & $0.006$ & $4403$ & $0.51$ \\
NGC3239 & 2 & $9.17$ & $-9.58$ & $0.932 \pm 0.793$ & $-0.047 \pm 0.231$ & $0.304$ & $-0.330$ & $1257$ & $0.33$ \\
NGC3351 & 1 & $10.37$ & $-10.25$ & $0.424 \pm 1.204$ & $0.356 \pm 0.332$ & $0.304$ & $0.227$ & $7080$ & $0.24$ \\
NGC3507 & 2 & $10.40$ & $-10.40$ & $0.838 \pm 0.267$ & $0.503 \pm 0.109$ & $0.517$ & $0.070$ & $30466$ & $0.54$ \\
NGC3511 & 2 & $10.03$ & $-10.12$ & $0.974 \pm 0.246$ & $0.366 \pm 0.091$ & $0.446$ & $-0.068$ & $19751$ & $0.75$ \\
NGC3521 & 2 & $11.02$ & $-10.45$ & $0.976 \pm 0.135$ & $0.648 \pm 0.073$ & $0.730$ & $-0.065$ & $103581$ & $0.88$ \\
NGC3596 & 2 & $9.66$ & $-10.18$ & $0.785 \pm 0.192$ & $0.650 \pm 0.090$ & $0.659$ & $0.133$ & $21993$ & $0.69$ \\
NGC3621 & 2 & $10.06$ & $-10.06$ & $1.010 \pm 0.128$ & $0.654 \pm 0.073$ & $0.801$ & $-0.155$ & $97443$ & $0.76$ \\
NGC3626 & 2 & $10.46$ & $-11.13$ & $0.794 \pm 0.377$ & $0.475 \pm 0.121$ & $0.446$ & $0.122$ & $3168$ & $0.75$ \\
NGC3627 & 1 & $10.84$ & $-10.25$ & $1.014 \pm 0.169$ & $0.863 \pm 0.111$ & $0.872$ & $-0.020$ & $24320$ & $0.75$ \\
NGC4254 & 1 & $10.42$ & $-9.93$ & $1.145 \pm 0.204$ & $0.703 \pm 0.108$ & $0.730$ & $-0.132$ & $20130$ & $0.81$ \\
NGC4298 & 2 & $10.02$ & $-10.36$ & $0.624 \pm 0.173$ & $0.586 \pm 0.070$ & $0.517$ & $0.264$ & $25588$ & $0.75$ \\
NGC4303 & 1 & $10.51$ & $-9.78$ & $0.964 \pm 0.209$ & $0.703 \pm 0.120$ & $0.801$ & $-0.068$ & $16580$ & $0.69$ \\
NGC4321 & 1 & $10.75$ & $-10.20$ & $1.080 \pm 0.215$ & $0.789 \pm 0.110$ & $0.659$ & $0.078$ & $26681$ & $0.63$ \\
NGC4424 & 2 & $9.91$ & $-10.43$ & $1.052 \pm 0.178$ & $0.553 \pm 0.102$ & $0.801$ & $-0.289$ & $3695$ & $0.59$ \\
NGC4457 & 2 & $10.42$ & $-10.93$ & $0.565 \pm 0.349$ & $0.784 \pm 0.145$ & $0.588$ & $0.452$ & $9790$ & $0.40$ \\
NGC4496A & 2 & $9.53$ & $-9.74$ & $0.698 \pm 0.385$ & $0.273 \pm 0.123$ & $0.446$ & $-0.038$ & $8446$ & $0.43$ \\
NGC4535 & 1 & $10.54$ & $-10.20$ & $1.111 \pm 0.325$ & $0.685 \pm 0.120$ & $0.517$ & $0.111$ & $8582$ & $0.55$ \\
NGC4536 & 2 & $10.40$ & $-9.86$ & $1.092 \pm 0.144$ & $0.779 \pm 0.080$ & $0.730$ & $-0.017$ & $20165$ & $0.69$ \\
NGC4540 & 2 & $9.79$ & $-10.56$ & $0.819 \pm 0.223$ & $0.592 \pm 0.105$ & $0.588$ & $0.111$ & $11515$ & $0.56$ \\
NGC4548 & 2 & $10.69$ & $-10.97$ & $0.794 \pm 0.329$ & $0.562 \pm 0.122$ & $0.446$ & $0.208$ & $11678$ & $0.51$ \\
NGC4569 & 2 & $10.81$ & $-10.68$ & $0.720 \pm 0.127$ & $0.804 \pm 0.066$ & $0.659$ & $0.330$ & $23275$ & $0.62$ \\
NGC4571 & 2 & $10.09$ & $-10.63$ & $0.466 \pm 0.349$ & $0.410 \pm 0.113$ & $0.375$ & $0.235$ & $16364$ & $0.28$ \\
NGC4579 & 2 & $11.15$ & $-10.81$ & $0.674 \pm 0.186$ & $0.726 \pm 0.092$ & $0.659$ & $0.283$ & $40074$ & $0.54$ \\
NGC4654 & 2 & $10.57$ & $-9.99$ & $0.895 \pm 0.110$ & $0.835 \pm 0.069$ & $0.872$ & $0.055$ & $52112$ & $0.80$ \\
NGC4689 & 2 & $10.22$ & $-10.61$ & $0.756 \pm 0.227$ & $0.651 \pm 0.088$ & $0.517$ & $0.261$ & $32495$ & $0.65$ \\
NGC4694 & 2 & $9.86$ & $-10.66$ & $0.979 \pm 0.156$ & $0.458 \pm 0.079$ & $0.659$ & $-0.188$ & $1860$ & $0.55$ \\
NGC4731 & 2 & $9.48$ & $-9.70$ & $0.715 \pm 0.235$ & $0.199 \pm 0.090$ & $0.517$ & $-0.170$ & $4385$ & $0.52$ \\
NGC4781 & 2 & $9.64$ & $-9.96$ & $0.955 \pm 0.155$ & $0.434 \pm 0.073$ & $0.659$ & $-0.195$ & $27874$ & $0.81$ \\
NGC4826 & 2 & $10.24$ & $-10.93$ & $0.798 \pm 0.139$ & $0.970 \pm 0.083$ & $0.872$ & $0.274$ & $20907$ & $0.84$ \\
NGC4941 & 2 & $10.17$ & $-10.53$ & $0.290 \pm 1.000$ & $0.187 \pm 0.222$ & $0.233$ & $0.120$ & $4679$ & $0.24$ \\
NGC4951 & 2 & $9.79$ & $-10.24$ & $0.974 \pm 0.386$ & $0.250 \pm 0.124$ & $0.375$ & $-0.115$ & $5225$ & $0.65$ \\
NGC5042 & 2 & $9.90$ & $-10.12$ & $0.833 \pm 0.504$ & $0.219 \pm 0.153$ & $0.375$ & $-0.093$ & $12488$ & $0.42$ \\
NGC5068 & 1 & $9.41$ & $-9.97$ & $0.919 \pm 0.625$ & $0.373 \pm 0.243$ & $0.517$ & $-0.102$ & $12231$ & $0.35$ \\
NGC5134 & 2 & $10.41$ & $-10.75$ & $0.744 \pm 0.290$ & $0.423 \pm 0.119$ & $0.517$ & $0.038$ & $15980$ & $0.51$ \\
NGC5248 & 2 & $10.41$ & $-10.05$ & $0.926 \pm 0.150$ & $0.832 \pm 0.080$ & $0.801$ & $0.091$ & $63197$ & $0.78$ \\
NGC5643 & 2 & $10.34$ & $-9.92$ & $0.769 \pm 0.161$ & $0.698 \pm 0.098$ & $0.801$ & $0.083$ & $99320$ & $0.67$ \\
NGC6300 & 2 & $10.47$ & $-10.19$ & $0.840 \pm 0.194$ & $0.731 \pm 0.087$ & $0.730$ & $0.117$ & $67368$ & $0.66$ \\
NGC7456 & 2 & $9.64$ & $-10.08$ & $0.636 \pm 0.067$ & $-0.179 \pm 0.002$ & $0.090$ & $-0.237$ & $922$ & $0.19$ \\
NGC7496 & 1 & $10.00$ & $-9.65$ & $0.985 \pm 0.352$ & $0.371 \pm 0.126$ & $0.446$ & $-0.069$ & $4023$ & $0.59$ \\
\cutinhead{$I_\mathrm{CO(2-1)}$ vs F335M$_\mathrm{PAH}$}
IC5332 & 1 & $9.68$ & $-10.07$ & $0.266 \pm 3.333$ & $0.380 \pm 0.596$ & $-0.700$ & $0.566$ & $1307$ & $0.11$ \\
NGC0628 & 1 & $10.34$ & $-10.10$ & $0.445 \pm 0.294$ & $0.741 \pm 0.095$ & $-0.500$ & $0.963$ & $2616$ & $0.34$ \\
NGC1087 & 1 & $9.94$ & $-9.83$ & $1.218 \pm 0.214$ & $0.721 \pm 0.079$ & $-0.300$ & $1.086$ & $6412$ & $0.73$ \\
NGC1300 & 1 & $10.62$ & $-10.55$ & $0.938 \pm 0.607$ & $0.720 \pm 0.138$ & $-0.600$ & $1.283$ & $596$ & $0.44$ \\
NGC1365 & 1 & $11.00$ & $-9.76$ & $1.000 \pm 0.768$ & $0.721 \pm 0.184$ & $-0.550$ & $1.271$ & $1335$ & $0.26$ \\
NGC1385 & 1 & $9.98$ & $-9.66$ & $0.942 \pm 0.123$ & $0.825 \pm 0.059$ & $-0.150$ & $0.966$ & $5778$ & $0.75$ \\
NGC1433 & 1 & $10.87$ & $-10.82$ & $0.854 \pm 0.974$ & $0.574 \pm 0.195$ & $-0.650$ & $1.130$ & $1160$ & $0.42$ \\
NGC1512 & 1 & $10.72$ & $-10.61$ & $0.776 \pm 1.698$ & $0.507 \pm 0.276$ & $-0.700$ & $1.050$ & $624$ & $0.43$ \\
NGC1566 & 1 & $10.79$ & $-10.13$ & $0.807 \pm 0.172$ & $1.085 \pm 0.093$ & $-0.150$ & $1.206$ & $7885$ & $0.52$ \\
NGC1672 & 1 & $10.73$ & $-9.85$ & $0.988 \pm 0.362$ & $0.874 \pm 0.121$ & $-0.400$ & $1.269$ & $3014$ & $0.50$ \\
NGC2835 & 1 & $10.00$ & $-9.90$ & $0.704 \pm 0.379$ & $0.579 \pm 0.108$ & $-0.500$ & $0.932$ & $1475$ & $0.46$ \\
NGC3351 & 1 & $10.37$ & $-10.25$ & $-0.121 \pm 126.184$ & $0.282 \pm 24.668$ & $-0.750$ & $0.191$ & $452$ & $0.14$ \\
NGC3627 & 1 & $10.84$ & $-10.25$ & $1.019 \pm 0.157$ & $1.088 \pm 0.083$ & $-0.150$ & $1.241$ & $18505$ & $0.66$ \\
NGC4254 & 1 & $10.42$ & $-9.93$ & $0.826 \pm 0.150$ & $1.092 \pm 0.071$ & $-0.250$ & $1.299$ & $10263$ & $0.68$ \\
NGC4303 & 1 & $10.51$ & $-9.78$ & $0.546 \pm 0.142$ & $1.109 \pm 0.070$ & $-0.250$ & $1.246$ & $2285$ & $0.54$ \\
NGC4321 & 1 & $10.75$ & $-10.20$ & $0.833 \pm 0.192$ & $1.088 \pm 0.071$ & $-0.350$ & $1.379$ & $2621$ & $0.55$ \\
NGC4535 & 1 & $10.54$ & $-10.20$ & $0.826 \pm 0.471$ & $0.881 \pm 0.118$ & $-0.550$ & $1.336$ & $1118$ & $0.45$ \\
NGC5068 & 1 & $9.41$ & $-9.97$ & $0.913 \pm 0.459$ & $0.539 \pm 0.146$ & $-0.450$ & $0.950$ & $4319$ & $0.37$ \\
NGC7496 & 1 & $10.00$ & $-9.65$ & $0.773 \pm 0.423$ & $0.557 \pm 0.110$ & $-0.550$ & $0.982$ & $797$ & $0.44$ \\
\cutinhead{$I_\mathrm{CO(2-1)}$ vs F1130W}
IC5332 & 1 & $9.68$ & $-10.07$ & $0.456 \pm 1.076$ & $0.341 \pm 0.265$ & $0.387$ & $0.165$ & $9230$ & $0.20$ \\
NGC0628 & 1 & $10.34$ & $-10.10$ & $0.768 \pm 0.258$ & $0.540 \pm 0.107$ & $0.624$ & $0.060$ & $13252$ & $0.58$ \\
NGC1087 & 1 & $9.94$ & $-9.83$ & $1.216 \pm 0.194$ & $0.504 \pm 0.091$ & $0.862$ & $-0.544$ & $9792$ & $0.75$ \\
NGC1300 & 1 & $10.62$ & $-10.55$ & $0.873 \pm 0.368$ & $0.492 \pm 0.133$ & $0.565$ & $-0.001$ & $4496$ & $0.48$ \\
NGC1365 & 1 & $11.00$ & $-9.76$ & $1.431 \pm 0.307$ & $0.758 \pm 0.157$ & $0.743$ & $-0.305$ & $11519$ & $0.49$ \\
NGC1385 & 1 & $9.98$ & $-9.66$ & $1.055 \pm 0.158$ & $0.542 \pm 0.099$ & $0.981$ & $-0.492$ & $11230$ & $0.76$ \\
NGC1433 & 1 & $10.87$ & $-10.82$ & $1.209 \pm 0.299$ & $0.544 \pm 0.120$ & $0.624$ & $-0.211$ & $9508$ & $0.44$ \\
NGC1512 & 1 & $10.72$ & $-10.61$ & $0.913 \pm 0.409$ & $0.342 \pm 0.120$ & $0.446$ & $-0.066$ & $4395$ & $0.47$ \\
NGC1566 & 1 & $10.79$ & $-10.13$ & $1.023 \pm 0.195$ & $0.775 \pm 0.131$ & $0.981$ & $-0.229$ & $31090$ & $0.61$ \\
NGC1672 & 1 & $10.73$ & $-9.85$ & $1.284 \pm 0.254$ & $0.604 \pm 0.132$ & $0.803$ & $-0.427$ & $9569$ & $0.67$ \\
NGC2835 & 1 & $10.00$ & $-9.90$ & $0.892 \pm 0.383$ & $0.351 \pm 0.148$ & $0.624$ & $-0.206$ & $12212$ & $0.42$ \\
NGC3351 & 1 & $10.37$ & $-10.25$ & $0.376 \pm 0.739$ & $0.269 \pm 0.207$ & $0.446$ & $0.101$ & $9418$ & $0.26$ \\
NGC3627 & 1 & $10.84$ & $-10.25$ & $1.157 \pm 0.152$ & $0.831 \pm 0.089$ & $1.040$ & $-0.373$ & $24603$ & $0.76$ \\
NGC4254 & 1 & $10.42$ & $-9.93$ & $1.161 \pm 0.165$ & $0.671 \pm 0.091$ & $0.862$ & $-0.329$ & $20433$ & $0.83$ \\
NGC4303 & 1 & $10.51$ & $-9.78$ & $0.986 \pm 0.179$ & $0.669 \pm 0.112$ & $0.921$ & $-0.240$ & $16929$ & $0.74$ \\
NGC4321 & 1 & $10.75$ & $-10.20$ & $1.140 \pm 0.244$ & $0.699 \pm 0.109$ & $0.743$ & $-0.149$ & $28405$ & $0.69$ \\
NGC4535 & 1 & $10.54$ & $-10.20$ & $1.021 \pm 0.257$ & $0.640 \pm 0.102$ & $0.624$ & $0.002$ & $10486$ & $0.57$ \\
NGC5068 & 1 & $9.41$ & $-9.97$ & $0.941 \pm 0.615$ & $0.342 \pm 0.256$ & $0.624$ & $-0.246$ & $14081$ & $0.36$ \\
NGC7496 & 1 & $10.00$ & $-9.65$ & $1.051 \pm 0.261$ & $0.333 \pm 0.098$ & $0.565$ & $-0.260$ & $4541$ & $0.64$ \\
\enddata
\tablecomments{
Columns: Cycle --- Indicates whether the galaxy was observed as part of Cycle 1 (GO 2107) or Cycle 2 (GO 3707); $\log_{10} M_\star$ --- global stellar mass [M$_\odot$]; $\log_{10} \mathrm{SFR}/M_\star$ global specific star formation rate [yr$^{-1}$]; $m$, $b$, $x_0$ --- best fit power law scaling parameters following Equation~\ref{eq:line} relating CO(2-1) to intensity in band $X$; $C_\mathrm{band}$ --- the normalization of the best-fit relation at $I_\nu^X=1$~MJy~sr$^{-1}$ [K~km~s$^{-1}$ (MJy sr$^{-1}$)$^{-1}$];
$N_{\rm pix}$ --- number of sight lines entering the analysis, where approximately four sight lines correspond to one independent measurements; $r$ --- rank correlation between CO(2-1) and intensity in band $X$ for all sight lines.
}
\end{deluxetable*}


==> gal_table_bottom.tex <==
\tablecomments{
Columns: $X$ --- JWST band compared to CO(2-1); $N_{\rm gal}$ --- number of galaxies entering this analysis; $N_{\rm pix}$ --- number of sightlines with $I_{\rm F770W}^{\rm PAH}$ entering correlation analysis; $\log_{10} \mathrm{CO}/X$ --- $\log_{10}$ of median ratio of CO(2-1) in K km s$^{-1}$ to intensity in MJy sr$^{-1}$ in band $X$ with error indicating the scatter in the ratio estimated from the median absolute deviation; $r$ --- rank correlation between CO(2-1) and intensity in band $X$ for all sightlines; $b$, $m$, $x_0$ --- best fit power law scaling parameters following Equation~\ref{eq:line} relating CO(2-1) to intensity in band $X$; $\sigma$ --- rms scatter in dex of individual data about the best fit scaling relation, inferred via the median absolute deviation. 
}


==> gal_table_top.tex <==
\tablecaption{Fits to all pixels outside galaxy centers for each galaxy.}


==> table2.tex <==
\begin{deluxetable*}{lrrrrrrrr}
\label{tab:fits}
\tablecolumns{8}
\include{big_fit_table_top}
\tablehead{
\colhead{$X$} & \colhead{$N_\mathrm{gal}$} & \colhead{$N_\mathrm{pix}$\tablenotemark{a}} & \colhead{$\log_{10}\mathrm{CO}/X$} & \colhead{$r$} & \colhead{$b$} & \colhead{$m$} & \colhead{$x_0$ } & \colhead{$\sigma$}}
\startdata
\cutinhead{All pixels}
F335M$_\mathrm{PAH}$ & 19 & 296834 & $1.27 \pm 0.38$ & $0.58$ & $1.38 \pm 0.07$ & $1.01 \pm 0.10$ & $0.10$ & $0.44$ \\
F770W$_\mathrm{PAH}$ & 70 & 2090731 & $0.03 \pm 0.35$ & $0.64$ & $1.39 \pm 0.06$ & $0.90 \pm 0.07$ & $1.44$ & $0.43$ \\
F770W & 70 & 2120025 & $-0.00 \pm 0.35$ & $0.64$ & $1.41 \pm 0.07$ & $0.91 \pm 0.07$ & $1.47$ & $0.43$ \\
F1130W & 20 & 972892 & $-0.12 \pm 0.37$ & $0.63$ & $1.20 \pm 0.08$ & $1.02 \pm 0.09$ & $1.34$ & $0.44$ \\
\cutinhead{All pixels outside of centers}
F335M$_\mathrm{PAH}$ & 19 & 279910 & $1.25 \pm 0.38$ & $0.56$ & $1.17 \pm 0.07$ & $1.04 \pm 0.12$ & $-0.05$ & $0.44$ \\
F770W$_\mathrm{PAH}$ & 70 & 2041245 & $0.02 \pm 0.35$ & $0.62$ & $1.12 \pm 0.07$ & $0.98 \pm 0.08$ & $1.16$ & $0.42$ \\
F770W & 70 & 2069574 & $-0.01 \pm 0.35$ & $0.62$ & $1.14 \pm 0.07$ & $0.99 \pm 0.08$ & $1.19$ & $0.42$ \\
F1130W & 20 & 946437 & $-0.12 \pm 0.37$ & $0.62$ & $0.93 \pm 0.08$ & $1.05 \pm 0.13$ & $1.11$ & $0.44$ \\
\cutinhead{All pixels in centers}
F335M$_\mathrm{PAH}$ & 17 & 16915 & $1.63 \pm 0.34$ & $0.80$ & $1.65 \pm 0.07$ & $0.78 \pm 0.09$ & $0.10$ & $0.41$ \\
F770W$_\mathrm{PAH}$ & 58 & 49469 & $0.18 \pm 0.33$ & $0.88$ & $1.52 \pm 0.07$ & $0.80 \pm 0.07$ & $1.44$ & $0.42$ \\
F770W & 58 & 50434 & $0.11 \pm 0.34$ & $0.87$ & $1.51 \pm 0.07$ & $0.83 \pm 0.07$ & $1.47$ & $0.44$ \\
F1130W & 18 & 26443 & $-0.02 \pm 0.30$ & $0.90$ & $1.30 \pm 0.07$ & $0.97 \pm 0.08$ & $1.34$ & $0.39$ \\
\cutinhead{All pixels in nebular regions (Cycle 1 only)}
F335M$_\mathrm{PAH}$ & 19 & 119051 & $1.19 \pm 0.33$ & $0.70$ & $1.13 \pm 0.07$ & $1.09 \pm 0.12$ & $-0.05$ & $0.39$ \\
F770W$_\mathrm{PAH}$ & 19 & 186605 & $-0.02 \pm 0.34$ & $0.75$ & $1.02 \pm 0.09$ & $1.03 \pm 0.11$ & $1.09$ & $0.40$ \\
F770W & 19 & 187137 & $-0.04 \pm 0.34$ & $0.75$ & $1.03 \pm 0.08$ & $1.06 \pm 0.11$ & $1.12$ & $0.40$ \\
F1130W & 19 & 194681 & $-0.17 \pm 0.33$ & $0.76$ & $0.89 \pm 0.08$ & $1.06 \pm 0.12$ & $1.11$ & $0.40$ \\
\cutinhead{All pixels in diffuse regions (Cycle 1 only)}
F335M$_\mathrm{PAH}$ & 19 & 160845 & $1.31 \pm 0.40$ & $0.44$ & $0.95 \pm 0.12$ & $1.28 \pm 0.32$ & $-0.40$ & $0.46$ \\
F770W$_\mathrm{PAH}$ & 19 & 632119 & $0.08 \pm 0.38$ & $0.52$ & $0.72 \pm 0.13$ & $1.20 \pm 0.27$ & $0.66$ & $0.47$ \\
F770W & 19 & 642906 & $0.05 \pm 0.38$ & $0.52$ & $0.74 \pm 0.13$ & $1.21 \pm 0.28$ & $0.70$ & $0.47$ \\
F1130W & 19 & 727342 & $-0.11 \pm 0.38$ & $0.54$ & $0.68 \pm 0.12$ & $1.22 \pm 0.25$ & $0.81$ & $0.47$ \\
\enddata
\include{big_fit_table_bottom}
\end{deluxetable*}


==> table_medrats.tex <==







\begin{deluxetable}{lrrr}[t]\label{tab:medrats}
 \tablecaption{Median $\log_{10}$ CO-to-MIR band ratios in units of K~km~s$^{-1}$/(MJy~sr$^{-1}$.}
    \tablehead{
         \colhead{Quantity} &  \colhead{Centers} & \colhead{Nebular} & \colhead{Diffuse} }
\startdata
CO/F335M & 0.48 & 0.40 & 0.47 \\
CO/F335M$_\mathrm{PAH}$ & 0.38 & 0.42 & 0.57 \\
CO/F770W$_\mathrm{PAH}$ &  0.31 & 0.35 & 0.40 \\
CO/F770W & 0.31 & 0.35 & 0.39 \\
CO/F1000W & 0.32 & 0.34 & 0.39 \\
CO/F1130W & 0.30 & 0.33 & 0.38 \\
CO/F2100W &  0.36 & 0.39 & 0.39 \\
\enddata
\end{deluxetable}




\begin{deluxetable}{lrrr}[t]
 \tablecaption{Median absolute deviation of CO-to-MIR band ratios [dex].}
    \tablehead{
         \colhead{Quantity} &  \colhead{Centers} & \colhead{Nebular} & \colhead{Diffuse} }
\startdata
CO/F335M & 0.71 & 0.45 & 0.16 \\
CO/F335M$_\mathrm{PAH}$ & 0.81 & 0.53 & 0.27 \\
CO/F770W$_\mathrm{PAH}$ & 0.86 & 0.76 & 0.50 \\
CO/F770W &0.85 & 0.76 & 0.50 \\
CO/F1000W & 0.85 & 0.76 & 0.54 \\
CO/F1130W &  0.86 & 0.77 & 0.54 \\
CO/F2100W & 0.84 & 0.75 & 0.53 \\
\enddata
\label{tab:madrats}
\end{deluxetable}



\begin{deluxetable}{lrrr}[t]
 \tablecaption{Pearson correlation coefficients between CO(2-1) and given MIR band, computed in $\log_{10}$ space.}
    \tablehead{
         \colhead{Quantity} &  \colhead{Centers} & \colhead{Nebular} & \colhead{Diffuse} }
\startdata
CO/F335M & 0.71 & 0.45 & 0.16 \\
CO/F335M$_\mathrm{PAH}$ & 0.81 & 0.53 & 0.27 \\
CO/F770W$_\mathrm{PAH}$ & 0.86 & 0.76 & 0.50 \\
CO/F770W & 0.85 & 0.76 & 0.50 \\
CO/F1000W & 0.85 & 0.76 & 0.54 \\
CO/F1130W  & 0.86 & 0.77 & 0.54 \\
CO/F2100W & 0.84 & 0.75 & 0.53 \\
\enddata
\label{tab:pearson}
\end{deluxetable}




\begin{deluxetable}{lrrr}[t]
 \tablecaption{Fits.}
    \tablehead{
         \colhead{Quantity} & \colhead{Centers} & \colhead{Nebular} & \colhead{Diffuse}}
\startdata
$x_0$ &  & & \\
$m$ &  & & \\
$b$ & & & \\
Median $\log_{10}$ CO/F770W & 0.31 & 0.35 & 0.40 \\
Scatter  & 0.86 & 0.76 & 0.50 \\
\enddata
\label{tab:fits}
\end{deluxetable}


